Hey there! You are using WhatsApp: Enumerating Three Billion Accounts for Security and Privacy

WhatsApp, with 3.5 billion active accounts as of early 2025, is the world's largest instant messaging platform. Given its massive user base, WhatsApp plays a critical role in global communication. To initiate conversations, users must first discover whether their contacts are registered on the platform. This is achieved by querying WhatsApp's servers with mobile phone numbers extracted from the user's address book (if they allowed access). This architecture inherently enables phone number enumeration, as the service must allow legitimate users to query contact availability. While rate limiting is a standard defense against abuse, we revisit the problem and show that WhatsApp remains highly vulnerable to enumeration at scale. In our study, we were able to probe over a hundred million phone numbers per hour without encountering blocking or effective rate limiting. Our findings demonstrate not only the persistence but the severity of this vulnerability. We further show that nearly half of the phone numbers disclosed in the 2021 Facebook data leak are still active on WhatsApp, underlining the enduring risks associated with such exposures. Moreover, we were able to perform a census of WhatsApp users, providing a glimpse on the macroscopic insights a large messaging service is able to generate even though the messages themselves are end-to-end encrypted. Using the gathered data, we also discovered the re-use of certain X25519 keys across different devices and phone numbers, indicating either insecure (custom) implementations, or fraudulent activity. In this updated version of the paper, we also provide insights into the collaborative remediation process through which we confirmed that the underlying rate-limiting issue had been resolved.

==> content/02_background.tex <==
\section{Background}

\subsection{Phone Number Formats}
The International Telecommunication Union (ITU) has established E.164\footnote{\url{https://www.itu.int/rec/T-REC-E.164/}} as an international phone numbering standard.
An allowed number consists of a country code (one to three digits) and a national telephone number.
In rare cases, multiple countries can share the same country code (e.g., US and CA both use +1). %
Although usually shorter, E.164 permits a maximum length of 15 digits for the complete international phone number.

Every country has its own national numbering scheme, that is defined and regulated by a regional entity being part of the ITU (e.g., the NANP).
In many countries, the first digits of the domestic number corresponds to a national routing code (also area code) that allows assigning a number to a specific geographic area or operator.
The residual digits of the domestic number represent the subscriber number.

The ITU publishes and maintains an overview of all country codes and national numbering plans of their members\footnote{\url{https://www.itu.int/oth/T0202.aspx?parent=T0202}}.
\gge{TODO: move links to other chapters and remove this chapter?}



